Inductive Synthesis of Inductive Heap Predicates -- Extended Version

We present an approach to automatically synthesise recursive predicates in Separation Logic (SL) from concrete data structure instances using Inductive Logic Programming (ILP) techniques. The main challenges to make such synthesis effective are (1) making it work without negative examples that are required in ILP but are difficult to construct for heap-based structures in an automated fashion, and (2) to be capable of summarising not just the shape of a heap (e.g., it is a linked list), but also the properties of the data it stores (e.g., it is a sorted linked list). We tackle these challenges with a new predicate learning algorithm. The key contributions of our work are (a) the formulation of ILP-based learning only using positive examples and (b) an algorithm that synthesises property-rich SL predicates from concrete memory graphs based on the positive-only learning. We show that our framework can efficiently and correctly synthesise SL predicates for structures that were beyond the reach of the state-of-the-art tools, including those featuring non-trivial payload constraints (e.g., binary search trees) and nested recursion (e.g., n-ary trees). We further extend the usability of our approach by a memory graph generator that produces positive heap examples from programs. Finally, we show how our approach facilitates deductive verification and synthesis of correct-by-construction code.

==> figure/tool.tex <==
% \begin{figure}[!htb]
% \setlength{\belowcaptionskip}{-10pt}
% \setlength{\abovecaptionskip}{5pt}
% \centering
% \resizebox{.45\textwidth}{!}{%
%     \footnotesize
%     \centering
%     \includegraphics[width=\textwidth]{figure/tool.pdf}%
% }
% \caption{Overview of \tool. User-provided inputs are in blue ovals;
%   plain-background rectangles are internal search parameters (our
%   additions are in bold font); blue rounded rectangles are
%   \popper's core components, orange one is new. \zy{no score any more}}
%     \label{fig:extended}
% \end{figure}


==> limit_and_future.tex <==
\section{Limitation and Future Work}
\label{sec:limit}

We have discussed some limitations of our approach in
\autoref{sec:fail} in the inductive predicate synthesis. Here we
discuss some other high-level limitations on the positive-only
learning and future works.

\paragraph{More on positive-only learning}


% Though we have mentioned that the positive-only learning is also applicable to other domains, we only discuss the issue of negative examples in  Separation Logic.
% Here we show different scenarios where (considerate) negative examples are not easy to obtain out of the context of Separation Logic.
% \begin{itemize}
%   \item \emph{Scenario 1:} To know what are the features on friendship among a group of people, we can ask them to fill a questionnaire about who are their friends. However, a questionnaire about who are \emph{not} their friends will not be an easy one to answer.
%   \item \emph{Scenario 2:} To learn the property of isosceles triangles, negative examples are not hard to provide; but if all negative examples provided are scalene, the learned predicates can be the property of equilateral triangles, which is not wrong but not specific enough.
% \end{itemize}

% It is both intuitive and supported by data that negation is not as
% welcomed as positive one. In daily knowledge representation,
% statements like "a tiger is an animal" are more common than "water is
% not an animal"; \citet{hossain2022analysis} conclude that negation is
% even less common in natural language understanding corpora than
% general-purpose English (22.6\%-29.9\%). Therefore, we believe that
% the positive-only learning can be a more practical setting for many
% applications.

Some basic assumptions of our positive-only learning restrict the
extension to more general settings. For example, noisy tolerance is
something not applicable to our current approach, because we need to
guarantee that the learned predicates are valid for all provided
examples. It is to be explored on whether the specificity can be
defined in other settings like probabilistic
ILP~\cite{de2008probabilistic} or differentiable
ILP~\cite{evans2018learning}.


\paragraph{Domain refinement and theory-based learning}

Since the learning domain of \popper is the definite clause, though we
have already encoded large number of SL-specific constraints in the ASP
encoding, either the hypothesis generation or the hypothesis testing
can be further refined. For example, the pure and spatial part of SL
predicates can be learned incrementally as the multilist example in
\autoref{sec:evaluation}. However, the encoding makes it hard to do
the incremental efficient.

Another direction is to use the theory-based learning approach. See in
most existing synthesisers, SMT solver is used to check the validity
of the candidate predicates. In our current synthesis, the search
space is traversed without awareness of the memory graphs' concrete
data, which is inherited from \popper. The good point of data
unawareness is to make less assumption on the input memory graphs: in
a real memory heap, some pointers can point to certain location which
is part of a data structure, but the pointer itself are not
necessarily to be part of the data structure though with reachability.
If we can have the assumption that the pointers with reachability is
of one data structure, we can use data-aware search to accelerate the
search.

